Robust Control Barrier-Value Functions for Safety-Critical Control

This paper works towards unifying two popular approaches in the safety control community: Hamilton-Jacobi (HJ) reachability and Control Barrier Functions (CBFs). HJ Reachability has methods for direct construction of value functions that provide safety guarantees and safe controllers, however the online implementation can be overly conservative and/or rely on chattering bang-bang control. The CBF community has methods for safe-guarding controllers in the form of point-wise optimization using quadratic programs (CBF-QP), where the CBF-based safety certificate is used as a constraint. However, finding a valid CBF for a general dynamical system is challenging. This paper unifies these two methods by introducing a new reachability formulation inspired by the structure of CBFs to construct a Control Barrier-Value Function (CBVF). We verify that CBVF is a viscosity solution to a novel Hamilton-Jacobi-Isaacs Variational Inequality and preserves the same safety guarantee as the original reachability formulation. Finally, inspired by the CBF-QP, we propose a QP-based online control synthesis for systems affine in control and disturbance, whose solution is always the CBVF's optimal control signal robust to bounded disturbance. We demonstrate the benefit of using the CBVFs for double-integrator and Dubins car systems by comparing it to previous methods.

==> legacy/sec_FTTV_robust_CBF.tex <==
\section{Finite-time Time-varying Robust Control Barrier-Value Functions (FTR-\CBVF) \shnote{Is it redundant to say both finite-time and time-varying? I'm not sure.} \label{sec:CBVF}}

\shnote{In this section we introduce the notion of a Finite-time time-varying robust control-barrier value function (FTR-\CBVF), and we demonstrate how the online algorithm used in the CBF community can be extended and brought to the HJ reachability community.}

\subsection{Defining the Control Barrier-Value Function}
% \textcolor{blue}{Donggun: I think the most of the theories in this section works for $x$ where the gradient of $B$ exists. Section V introduces a viscosity theory which supports that the definition of FTR CBF may not require differentiability for all $x$ but almost everywhere. 
% Also, I have been checked the Craig Evans' book that usually first states the viscosity theory, and then, for example, \eqref{eq:FTR-CBF} is stated for $x$ at which $B$ is differentiable as a remark. 
% Also, the viscosity theory that we know is for equations but not for inequalities. Using this knowledge, we cannot say both super- and sub-solutions for the viscosity theory, but we only can say about super-solution (but not sub-solution).
% \\
% Thus, I suggest the following orders. 1) Section V's viscosity theory comes first and then makes readers have sense that $V$ is the maximal CBF, that is continuous and  differentiable almost everywhere. Thus, 'differentiable almost everywhere' makes sense in the definition of FTR-CBF. 2) And then for $x$ at which $B$ (or $V$) is differentiable, all stuffs in Section IV can be stated.
% }

\begin{definition}
\label{def:FTR-CBF}
\shnote{I'm changing macro for the CBVF here so we can put in whatever notation we want to distinguish it from a normal CBF}
Consider $\BV(x, t):\LL \times [T, 0] \rightarrow \R$, for some $t  < 0$, \jc{which is Lipschitz continuous in $x$ and Lipschitz continuous and differentiable in $t$}. Super-zero level sets of $\BV$, $\mathcal{C}(t):=\{x\in\R^n : \BV(x, t) \ge 0\}$, should be non-empty and satisfy $\mathcal{C}(t) \subset \LL$ for all $t\in[T, 0]$. $\BV$ is a Finite-time Time-varying Robust Control Barrier-Value Function (FTR-\CBVF) if there exists an extended class $\mathcal{K}_\infty$ function $\alpha$ such that

\small
\begin{equation}
D_{t} \BV(x, t) + \max_{\ctrl\in \cset} \min_{\dstb \in \dset} D_{x} \BV(x, t) \cdot f(x, \ctrl, \dstb) \geq  -\alpha(\BV(x, t)) \label{eq:FTR-CBF}
\end{equation}
\normalsize

\noindent for all $x\in\mathcal{C}(t)$ where the gradient exists for all $t\in[T, 0]$. 
\end{definition}

The FTR-\CBVF~ defined by Definition \ref{def:FTR-CBF} will satisfy the following property:

\begin{theorem}
\label{th:FTR-CBF-safety}
For FTR-\CBVF~ $\BV$ and the extended class $\mathcal{K}_\infty$ function $\alpha$ that satisfies Definition \ref{def:FTR-CBF}, for any initial state $x\in \mathcal{C}(T)$, you can always find an admissible control signal $\ctrl(\cdot) \in \cfset_{[T, 0]}$ that $\ctrl(t)$ satisfies

\small
\begin{align}
    D_{t} \BV(\state(t), t) + \min_{\dstb \in \dset} D_{x} \BV(\state(t), t) \cdot f(\state(t), \ctrl(t), \dstb) & \nonumber \\
    \geq  -\alpha(\BV(\state(t), t)) & \label{eq:FTR-CBF-constraint}
\end{align}
\normalsize

\noindent for $\forall t\in[T, 0]$ when $D_{x}\BV(\state(t),t)$ exists. \shnote{what do we want to say about the gradient existing here?} The resulting trajectory $\state(s)$ which solves \eqref{eq:system} for $(x, T, \ctrl, \strategy[\ctrl])$ will be safe for all $t\in[T, 0]$, i.e.  $\state(t)\in \LL$, for any $\strategy\in\Strategy_{[t, 0]}$. 
\end{theorem}
\begin{proof}
\jc{(Redo the proof. How do we deal with $\strategy$?)} For any initial state $x\in \mathcal{C}(t)$ and disturbance signal $\dstb(\cdot)\in\dfset_{[t, 0]}$, the control signal $\ctrl(s)$ and the corresponding trajectory $\trajsimple(s)$ is well defined, since we can always find $\ctrl(s)\in \cset$ that satisfies \eqref{eq:FTR-CBF-constraint} by Definition \ref{def:FTR-CBF}, and under such $\ctrl(s)$, $\trajsimple(s)\in\mathcal{C}(s)$ because

\small
\begin{align*}
    \dot{\BV}(\trajsimple(s), s) = D_{s} \BV(\trajsimple(s), s) + D_{x} \BV(\trajsimple(s), s) \cdot f(\trajsimple(s), \ctrl(s), \dstb(s)) & \\
    \geq  -\alpha(\BV(\trajsimple(s), s)) \quad \text{almost everywhere in}\;s\in[t, 0] &
\end{align*}
\begin{equation*}
\Rightarrow \BV(\trajsimple(s)) \ge 0 \quad \text{for all}\;s\in[t, 0].
\end{equation*}
\normalsize
Therefore, $\trajsimple(s)$ is well defined as well for $s\in[t, 0]$, and it is safe (i.e. $\trajsimple(s)\in\LL$).
\end{proof}

Theorem \ref{th:FTR-CBF-safety} implies that if a FTR-\CBVF~ $\BV$ exists \shnote{and is differentiable in x?}, we can guarantee safety for all $x \in \mathcal{C}(T)$ for the time interval $[T, 0]$, even under the worst-case disturbance.

\shnote{Some remark on how we're not calling this a CBF directly because of that whole controller continuity in the state space thing}


==> legacy/sec_cbf_reachability.tex <==
\section{Connection between HJ Reachability and CBF}
\label{sec:cbf_hj}
\begin{figure}%[!htb]
\centering
\includegraphics[width=0.5\textwidth]{figures/main_diagram_new.png}
\caption{Geometric connection between the viability kernel and the CBF's super-zero level set. The gray region represents the failure set that the system should not enter. The constraint set is therefore the complement $\LL$, seen in white. On the left, the infinite-time viability kernal generated by HJ reachability is shown in blue, with the CBF safe set a guaranteed under-approximation. On the right, the finite-time viability kernel is generally larger than the infinite-time version, as there exists more states that can be safe for only a finite time horizon. \shnote{not sure if we can say this next sentence in the conference version} This viability kernel is the maximal robust CBF safe set. \shnote{This figure is blurry to me. maybe try saving as a pdf. Also label constraint set $\LL$ in the white area}}
\label{fig:main-diagram}
\vspace{-10pt}
\end{figure}

In this section, we analyze a formal connection between HJ reachability analysis and CBF based safety analysis. \shnote{is this still a ``formal'' connection?} Figure~\ref{fig:main-diagram} provides a visualization of the comparison in this section. 

Note that CBFs provides infinite-time safety guarantee from Theorem \ref{th:cbf}. Therefore, we start by introducing HJ reachability analysis for the infinite-horizon case. To explain this, first we define a desirable property of a set:
\begin{definition}
\textbf{Robust Control Invariance: }A nonempty set $\mathcal{I} \subset \R^{n}$ is robust control invariant if for every $x \in \mathcal{I}$, if there exists a control signal $\ctrl\in\cfset_{[0, \infty)}$ such that for any $\strategy \in \Strategy_{[0, \infty)}$, $\state(s)$ that solves \eqref{eq:system} for $(x, 0, \ctrl, \strategy[\ctrl])$ satisfies
\begin{equation}
    \state(s) \in \mathcal{I} \;\; \forall s \in [0, \infty).
\end{equation}
\end{definition}

This is a generalization of the notion of control invariance under the disturbance effect. Given a robust control invariant set $\mathcal{I} \subset \LL$, we can always find a control that guarantees the trajectory to stay in $\mathcal{I}$ under the worst case disturbance, therefore rendering the trajectory safe for infinite time. The next question is how to find such a set $\mathcal{I}$ and the corresponding control policy that satisfies the robust control invariance. First, define the infinite horizon value function as
\begin{equation}
\label{eq:v_infty}
    \VV_{\infty}(x)\!:=\!\lim_{t\rightarrow-\infty}\VV(x, t)\!=\!\inf_{\strategy\in\Strategy_{[0,\infty)}} \sup_{\ctrl \in \cfset_{[0,\infty)}} \inf_{s \in [0, \infty)} \lf(\state(s))
\end{equation}
\shnote{I'm confused about the direction of time in the above equation.} where $\state(\cdot)$ that solves \eqref{eq:system} for $(x, 0, \ctrl, \strategy[\ctrl])$. $\VV_\infty$ is locally bounded on $\R^n$ and it is a viscosity solution of the stationary HJI-VI \cite{fialho_worst}
\begin{align}
\label{eq:hji-vi-invariant}
    0=\min\{\lf(x)-\VV_\infty(x),\max_{\ctrl\in \cset} \min_{\dstb\in \dset} D_x \VV_\infty (x)\cdot f(x,\ctrl,\dstb)\}.
\end{align}
Then, maximal robust control invariant set contained in $\LL$ can be verified as the super-zero level set of $V_{\infty}(x)$ by the following proposition. \shnote{has no one proved this before? Could we just cite something instead of doing the proof?} % \jc{However, the existence of well-defined  $V_{\infty}(x)$ is hard to verify in general.}

\begin{proposition}
\label{prop:max_control_invariant_set}
$\Safe_{\infty} := \{ x : V_{\infty}(x) \geq 0 \}$ is the maximal robust control invariant set contained in $\LL$; any set strictly containing $\Safe_{\infty}$ and contained in $\mathcal{L}$ is not robust control invariant.
\end{proposition}

\begin{proof} 
In the following proof, $\state$ solves \eqref{eq:system} for $(x, 0, \ctrl, \strategy[\ctrl])$.
First, we prove that the set $\Safe_{\infty}$ is robust control invariant and contained in $\LL$. For all $x \in \Safe_{\infty} = \{ x : \VV_{\infty}(x) \geq 0 \}$,

\small
\begin{equation*}
\begin{aligned}
& V_{\infty}(x)  \geq 0 \iff \forall \strategy \in \Strategy_{[0, \infty)},\;\; \sup_{\ctrl \in \cfset_{[0,\infty)}} \inf_{s \in [0, \infty)} \lf(\state(s)) \geq 0\\
& \iff \forall \strategy \in \Strategy_{[0, \infty)},\;\exists \ctrl \in \cfset_{[0,\infty)} \; s.t. \; \forall s \in [0, \infty), \; \state(s) \in \LL,
\end{aligned}
\end{equation*}
\normalsize

\noindent and
\small
\begin{equation*}
\lf(x) \geq \inf_{s \in [0, \infty)} \lf(\state^{*}(s)) = \VV_{\infty}(x)  \geq 0 \quad \forall \strategy \in \Strategy_{[0, \infty)}
\end{equation*}
\normalsize

\noindent where $\state^{*}$ solves \eqref{eq:system} for $(x, 0, u^{*}, \strategy[\ctrl^{*}])$ with $\ctrl^*$ the optimal control signal. Therefore, $\Safe_{\infty}$ is robust control invariant and contained in $\LL$.

Second, for all $x \in \{ x : \VV_{\infty}(x) < 0 \}$,

\small
\begin{equation}
\begin{aligned}
& \VV_{\infty}(x)  < 0 \iff \exists \strategy \in \Strategy_{[0, \infty)}, \sup_{\ctrl \in \cfset_{[0,\infty)}} \inf_{s \in [0, \infty)} \lf(\state(s)) < 0 \quad \\
& \iff \exists \strategy \in \Strategy_{[0, \infty)}, \forall \ctrl \in \cfset_{[0,\infty)}, \; \exists s \in [0, \infty)\; s.t. \; \state(s) \notin \LL.
\end{aligned}
\label{eq:th3part2}
\end{equation}
\normalsize
Consider a set $\mathcal{I}$ strictly containing $\Safe_{\infty}$ and contained in  $\LL$. There exists an element $x \in \mathcal{I},\; x \in \{ x : \VV_{\infty}(x) < 0 \}$. From (\ref{eq:th3part2}), any trajectory starting from $x$ will eventually exit $\LL$ under some disturbance strategy, and therefore also from $\mathcal{I}$, i.e. $\mathcal{I}$ is not robust control invariant.
\end{proof}


% \textcolor{blue}{Donggun: I realized that $\mathcal{S}_\infty\neq\{x~:~V_\infty(x)\geq 0\}$, in general, due to the supremum and infimum operations. To achieve the maximum and minimum, $U$ and $D$ need to be assumed as convex. The below proof assumes that $U$ and $D$ are convex.
% \\
% (Probably at the beginning of this paper) suppose $U$ and $D$ are convex. 
% A set of feasible state trajectories
% \begin{align}
%     X_{[t,\infty)}(x) = \{ \mathrm{x}~:~\dot{\mathrm{x}}(s)=f(\mathrm{x}(s),u(s),d(s)), \notag\\
%     \text{for } u\in\mathcal{U}_{[0,\infty)},d\in\mathcal{D}_{[0,\infty)}, \mathrm{x}(0)=x\}
% \end{align}
% is compact by \cite{altarovici2013general}.
% Thus, there exists the maximum control and minimum disturbance signals.
% \\
% And then, your argument is valid.
% } 


First, it is important to note the geometric connection between $\mathcal{C}$, the super-zero level set of the CBF $\BB$, and $\Safe_\infty$, the maximal control invariant set contained in $\LL$. In order to use $\BB$ for our safety objective \eqref{eq:safeset}, its super-zero level set $\mathcal{C}$ should be a subset of $\LL$, as shown in Fig.~\ref{fig:main-diagram}. Since $\mathcal{C}$ is a control invariant set, by Proposition \ref{prop:max_control_invariant_set}, $\mathcal{C} \subset \Safe_\infty$. Note that here we are considering systems without disturbance for both $\Safe_\infty$ and $\mathcal{C}$. The disturbance term will be introduced again in the next section.

\shnote{We're getting rid of this right?} Second, $V_{\infty}$ can be directly used as a CBF by the following proposition. 
% However, existence of $V_{\infty}$ is non-trivial for many systems as emphasized before.
% \begin{proposition}
% If $V_{\infty}(x) := \lim_{t\rightarrow-\infty}V(x, t)$ is well-defined in $\Safe_\infty$ for a controlled system without disturbance $\dot{\state}(s)\!=\!f(\state(s), u(s))$, then $V_{\infty}$ is a valid CBF for any extended class $\mathcal{K}_{\infty}$ function $\alpha$.\footnote{How to deal with the continuously differentiable property that the definition of CBF should satisfy? At the point where the value function is not differentiable, how do we choos the gradient?}
% \end{proposition}
% \begin{proof}
% For any $x \in \mathcal{S}_{\infty}=\{x \in \LL : V_{\infty}(x) \geq 0\}$,
% \begin{equation*}
%     \max_{u \in U}  D_{x}V_{\infty}(x) \cdot f(x, u)  \geq 0 \geq - \alpha(V_{\infty}(x)).
% \end{equation*}
% \end{proof}

\begin{proposition}
\label{prop:V_inf_is_valid_CBF}
% If $V_{\infty}(x) := \lim_{t\rightarrow-\infty}V(x, t)$ is a continuous viscosity solution to 
% \begin{align}
%     0=\min\{l(x)-V_\infty(x),\max_{u\in U} D_x V_\infty (x)\cdot f(x,u)\}, 
% \end{align}
% for $x\in\mathbb{R}^n$, 
% then, 
$V_{\infty}$ is a valid CBF for any extended class $\mathcal{K}_{\infty}$ function $\alpha$.
\end{proposition}
\begin{proof} Since $D_x \VV_\infty (x)$ exists a.e. in $\R^n$, 
\begin{equation*}
\max_{\ctrl\in U} D_x \VV_\infty(x)\cdot f(x,\ctrl)\geq 0    
\end{equation*}
for $x$ a.e. in $\R^n$.
Thus, \eqref{eq:cbf} holds for a.e. $x\in\mathcal{S}_\infty$ for any extended class $\mathcal{K}_{\infty}$ function $\alpha$.
\end{proof}




Several works has extended the concept of CBFs to robust versions \cite{ames_robust, jankovic} and time-varying version \cite{nguyen2016optimal, grandia2020cbf-legged_robots}, and the concept of finite-time safety is also tackled recently \cite{ohnishi2021constraint, fixed_time_bf}, however, under different characterizations and applications. Inspired by the reachability analysis, we begin next section by extending the concept of CBF to finite-time robust safety guarantee. 
